COLMAP-Free 3D Gaussian Splatting

While neural rendering has led to impressive advances in scene reconstruction and novel view synthesis, it relies heavily on accurately pre-computed camera poses. To relax this constraint, multiple efforts have been made to train Neural Radiance Fields (NeRFs) without pre-processed camera poses. However, the implicit representations of NeRFs provide extra challenges to optimize the 3D structure and camera poses at the same time. On the other hand, the recently proposed 3D Gaussian Splatting provides new opportunities given its explicit point cloud representations. This paper leverages both the explicit geometric representation and the continuity of the input video stream to perform novel view synthesis without any SfM preprocessing. We process the input frames in a sequential manner and progressively grow the 3D Gaussians set by taking one input frame at a time, without the need to pre-compute the camera poses. Our method significantly improves over previous approaches in view synthesis and camera pose estimation under large motion changes. Our project page is https://oasisyang.github.io/colmap-free-3dgs

==> algo_global.tex <==
\begin{algorithm}[th]
    \caption{COLMAP-Free 3DGS Optimization}
    \label{alg:global}
    \begin{algorithmic}
        \State $\{I_t | t=1...N\} \gets$ Image sequence
        \State $\text{DPT} \gets $ Monocular Depth Estimation Model
        \State $D_1 \gets \text{DPT}(I_1)$ 
        \State $G \gets$ InitGauss($I_1$, $D_1$) 
        \Comment{Init Globla Gauss}
        \State $i \gets 0$	\Comment{Iteration Count}
        % =\{P, C, R, S, O\} 
        \ForAll{Image $I_t$ \textbf{in} ${I_{t=1...N}}$}
            \State $T_t \gets $ Local 3DGS($I_t, I_{t+1}$) \Comment{Eestimate Pose}
            \While{not converged}
                \State $T_j, I_j \gets$ SampleTrainingView() \Comment{$j \leq t$}
                \State $\hat{I_{j}} \gets$ Rasterize($G$, $T_j$)
                \State $L \gets Loss(I_j, \hat{I}_j) $ 
                \State $G \gets$ Adam($\nabla L$)      \Comment{Update Gauss}
                \State $i \gets i+1$
            \EndWhile
            \ForAll{Gaussians $(\mu, \Sigma, c, \alpha)$ \textbf{in} $G$}
                \If{$\nabla_p L > \tau_p$} \Comment{Densification}
                    \State SplitGaussian($\mu, \Sigma, c, \alpha$)
                    \State CloneGaussian($\mu, \Sigma, c, \alpha$)
                    % \If{$\|S\| > \tau_S$}	\Comment{Over-reconstruction}
                    %     \State SplitGaussian($\mu, \Sigma, c, \alpha$)
                    % \Else    \Comment{Under-reconstruction}
                    %     \State CloneGaussian($\mu, \Sigma, c, \alpha$)
                    % \EndIf	
                \EndIf
                \If{$\alpha < \epsilon$ or IsTooLarge($\mu, \Sigma)$}	\Comment{Pruning}
                    \State RemoveGaussian()	
                \EndIf
            \EndFor
        \EndFor

        
        % \State $M \gets$ SfM Points	\Comment{Positions}
        % \State $S, C, A \gets$ InitAttributes() \Comment{Covariances, Colors, Opacities}
        % \State $i \gets 0$	\Comment{Iteration Count}
        
        % \While{not converged}
        
        % \State $V, \hat{I} \gets$ SampleTrainingView()	\Comment{Camera $V$ and Image}
        % \State $I \gets$ Rasterize($M$, $S$, $C$, $A$, $V$)	\Comment{Alg.~\ref{alg:rasterize}}
        
        % \State $L \gets Loss(I, \hat{I}) $ \Comment{Loss}
        
        % \State $M$, $S$, $C$, $A$ $\gets$ Adam($\nabla L$) \Comment{Backprop \& Step}
        
        
        % \If{IsRefinementIteration($i$)}
        % \ForAll{Gaussians $(\mu, \Sigma, c, \alpha)$ $\textbf{in}$ $(M, S, C, A)$}
        % \If{$\alpha < \epsilon$ or IsTooLarge($\mu, \Sigma)$}	\Comment{Pruning}
        % \State RemoveGaussian()	
        % \EndIf
        % \If{$\nabla_p L > \tau_p$} \Comment{Densification}
        % \If{$\|S\| > \tau_S$}	\Comment{Over-reconstruction}
        % \State SplitGaussian($\mu, \Sigma, c, \alpha$)
        % \Else								\Comment{Under-reconstruction}
        % \State CloneGaussian($\mu, \Sigma, c, \alpha$)
        % \EndIf	
        % \EndIf
        % \EndFor		
        % \EndIf
        % \State $i \gets i+1$
        % \EndWhile
    \end{algorithmic}
\end{algorithm}


==> figs/supp_co3d_nvs_part1.tex <==
\begin{figure*}[tp]
    \centering
    % \bgroup 
    %  \def\arraystretch{0.1} 
    %  \setlength\tabcolsep{25pt}
    %  \begin{tabular}{ccccc}
    %  BARF~\cite{lin2021barf} & SC-NeRF~\cite{jeong2021self} & Nope-NeRF~\cite{bian2023nope} & Ours & Ground-truth \\
    %  \end{tabular} \egroup
    % \includegraphics[width=1.0\linewidth]{figs/church_compare.pdf} \\
    % \includegraphics[width=1.0\linewidth]{figs/museum_compare.pdf} \\
    % \includegraphics[width=1.0\linewidth]{figs/family_compare.pdf} \\    
    % \vspace{-2mm}
    \includegraphics[width=0.95\linewidth]{figs/co3d_compare_supp_1.jpg}
    \caption{\textbf{Qualitative comparison for novel view synthesis on CO3D-V2.}}
    \label{fig:supp_co3d_nvs_part1}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

